PyTester: Deep Reinforcement Learning for Text-to-Testcase Generation

Test-driven development (TDD) is a widely-employed software development practice that mandates writing test cases based on requirements before writing the actual code. While writing test cases is the centerpiece of TDD, it is time-consuming, expensive, and often shunned by developers. To address these issues associated with TDD, automated test case generation approaches have recently been investigated. Such approaches take source code as input, but not the requirements. Therefore, existing work does not fully support true TDD, as actual code is required to generate test cases. In addition, current deep learning-based test case generation approaches are trained with one learning objective, i.e., to generate test cases that are exactly matched with the ground-truth test cases. However, such approaches may limit the model's ability to generate different yet correct test cases. In this paper, we introduce PyTester, a Text-to-Testcase generation approach that can automatically generate syntactically correct, executable, complete, and effective test cases while being aligned with a given natural language requirement. We evaluate PyTester on the public APPS benchmark dataset, and the results show that our Deep RL approach enables PyTester, a small language model, to outperform much larger language models like GPT3.5, StarCoder, and InCoder. Our findings suggest that future research could consider improving small over large LMs for better resource efficiency by integrating the SE domain knowledge into the design of reinforcement learning architecture.

==> sections/abstract.tex <==
\begin{abstract}
% In Test-Driven Development (TDD), software testing is the first essential steps to ensure the functional correctness of the source code according to the specification. 
% To write codes that are functionally correct to a specification, developers need to first design and write high-quality test cases.
% However, writing test cases requires effort and is tedious for developers.
% Previous research proposes approaches to automatically generating the test cases using search-based and deep learning based approaches.
% Nonetheless, the approaches are heuristic or learn solely from text-based similarity and not from functional correctness.
% Nonetheless, popular dynamically-type programming languages such as Python are still limited on this front.
Test-driven development (TDD) is a widely-employed software development practice that mandates writing test cases based on requirements \emph{before} writing the actual code.
While writing test cases is the centrepiece of TDD, it is time-consuming, expensive, and often shunned by developers. 
To address these issues associated with TDD, automated test case generation approaches have recently been investigated.
Such approaches take source code as input, but not the requirements.
Therefore, existing work does not fully support true TDD, as actual code is required to generate test cases. 
In addition, current deep learning-based test case generation approaches are trained with one learning objective, i.e., to generate test cases that are exactly matched with the ground-truth test cases.
However, such approaches may limit the model's ability to generate different yet correct test cases. 
In this paper, we introduce \ours, a Text-to-Testcase generation approach that can
automatically generate syntactically correct, executable, complete, and effective test cases while being aligned with a given natural language requirement.
We evaluate \ours~on the public APPS benchmark dataset, and the results show that our Deep RL approach enables \ours, a small language model, to outperform much larger language models like GPT3.5, StarCoder, and InCoder.
Our findings suggest that future research could consider improving small over large LMs for better resource efficiency by integrating the SE domain knowledge into the design of reinforcement learning architecture.

% is still not applicable to the TDD context.
% Our Deep RL-based model is optimized with Proximal Policy Optimization (PPO) on a reward function to generate syntactically correct and executable test cases with high code coverage and being aligned with the given requirement.
% Experimental results show that our \ours~model can generate test cases that achieve an average code coverage of 80.98\% and a mutation score of 61.45\%, which are 12\%-81\% and 7\%-61\% higher than three state-of-the-art large language models (LLMs): GPT3.5, StarCoder, and InCoder, respectively. 


% with different syntax and test inputs, while being syntactically correct, executable, and achieving high code coverage.
%  higher , 

%  the Code Coverage of  and the Mutation Score of 61.45\% on the ground truth code which is  more accurate than the baselines.
 

% outperforms all of the studied state-of-the-art LLMs 



% on every evaluation metric achieving the Code Coverage of 80.98\% and the Mutation Score of 61.45\% on the ground truth code which is 12\%-81\% and 7\%-61\% more accurate than the baselines.


% We conduct an intensive ablation study on functional-guided reward functions: the syntax parsing, test execution, and code coverage feedback, on .
% Then, we evaluate \ours~on four functional evaluation metrics against three state-of-the-art Large Language Models (LLMs): GPT3.5, StarCoder, and InCoder.
% As a result, \ours~outperforms all the state-of-the-art LLMs on every evaluation metric achieving the Code Coverage of 80.98\% and the Mutation Score of 61.45\% on the ground truth code which is 12\%-81\% and 7\%-61\% more accurate than the baselines.


% existing DL - the learning process aims to generate test cases in order to exactly match with the GT. 
% In reality, alternative test cases that do not match the groud-truth may also be possible 


% - GT test cases suboptimal - cannot capture all possibility of the test cases. learning process of existing work limited to the GT, inaccurate

% argue - generated test cases that are correct must be compilable, and executable (i.e., all test cases are passed the execution), while achieving high code coverage.

% traditional - learn only one objective - to match GT, 

% assert func(1,2) == 3
% assert 3 == func(1,2)

% test - input output



% lead to model overfitting (slight change in the input may produce completely different test cases). 

% generated test cases 




% however, in reality, alternative generated test cases that are not the same as the ground truth may be correct if they are compilable, executable, passing (aligned with the actual functionality of the code), and achieve high code coverage.





% without considering whether test cases are aligned with the requirements and also achieve high code coverage or not.



% However, in reality, the variation of the test cases -ok as long as it is aligned with the requirements.

% - previous approach - only code to test
% - search + DL - do not consider the code functionality - 

% Moreover, the input are heavily relied on implemented source code, and less on the natural language specification.
% Therefore, we propose \ours, a functional-guided Deep Reinforcement Learning model, for Python test case generation given a natural language specification.
% We conduct an intensive ablation study on functional-guided reward functions: the syntax parsing, test execution, and code coverage feedback, on the APPS dataset.
% Then, we evaluate \ours~on four functional evaluation metrics against three state-of-the-art Large Language Models (LLMs): GPT3.5, StarCoder, and InCoder.
% As a result, \ours~outperforms all the state-of-the-art LLMs on every evaluation metric achieving the Code Coverage of 80.98\% and the Mutation Score of 61.45\% on the ground truth code which is 12\%-81\% and 7\%-61\% more accurate than the baselines.
\end{abstract}
